Listening to the city, attentively: A Spatio-Temporal Attention Boosted Autoencoder for the Short-Term Flow Prediction Problem

In recent years, studying and predicting alternative mobility (e.g., sharing services) patterns in urban environments has become increasingly important as accurate and timely information on current and future vehicle flows can successfully increase the quality and availability of transportation services. This need is aggravated during the current pandemic crisis, which pushes policymakers and private citizens to seek social-distancing compliant urban mobility services, such as electric bikes and scooter sharing offerings. However, predicting the number of incoming and outgoing vehicles for different city areas is challenging due to the nonlinear spatial and temporal dependencies typical of urban mobility patterns. In this work, we propose STREED-Net, a novel deep learning network with a multi-attention (spatial and temporal) mechanism that effectively captures and exploits complex spatial and temporal patterns in mobility data. The results of a thorough experimental analysis using real-life data are reported, indicating that the proposed model improves the state-of-the-art for this task.

==> DataDescription.tex <==
%\vin{a me questa transizione non piace. Abbiamo parlato di un modello complesso, ora mi parli di dataset. Perché? I dataset servono per fare una sperimentazione, ma la sperimentazione non è ancora spiegata. Devi prima impostare la sperimentazione, poi definisci setup sperimentale (dataset + baseline).}
In this paper, different case studies were used to carry out the validation experiments of the proposed framework. In particular,\vin{e infatti qui mi parli di ``experiments''} these are three real-world datasets containing records of vehicle trajectories.%\vin{perché usiamo traiettorie? l'input al modello erano delle slice di in/out flows in regioni. NOn ci sono dataset già pronti? devi ricavare le slice da dataset di traiettorie? Lo spazio poi come lo suddividi? Immagino che NYC e BJ abbiano regioni di dimensioni differenti. O la dimensione è la stessa, e cambia il numero di regioni considerate? Queste domande possono trovare risposta solo dopo che hai definito cosa devi sperimentare}
\begin{enumerate}
    \item \textit{BikeNYC.} The bike trajectory dataset was collected by the \textit{NYC Bike system} in 2014 from April 1 to September 30. Records from the last 10 days form the testing dataset, while the rest is used for training. The length of each time period is of 1 hour.%\vin{cioè? cos'è un time period? stai dicendo che hai snapshot ogni ora? o che raccogli dati per un'ora?}
    \item \textit{TaxiBJ.} The taxi trajectory dataset in Beijing is divided into 4 different time periods: July 1 2013 - October 30 2013, March 1 2014 - June 30 2014, March 1 2015 - Jun 30 2015, November 1 2015 - April 15 2016. The last four weeks are test data and the others are used for training purposes. The length of each time period is set to 30 minutes.
    \item \textit{TaxiNYC.} Travel data, trajectories, taken by taxis in New York City. They were collected from January 1, 2009 to December 31, 2014. The last four weeks are test data and the others are used for training purposes. The length of each time period is set to one hour.
%    \item \textit{CarRoma.} Private vehicles equipped with an OBU %that %has three fundamental elements inside: a GPS receiver, an %accelerometer for crash detection and a GSM-GPRS module for %automatic or on-demand communication of stored data and positions %to the Service Center. The OBU 
%    performs functions of recording the use of the vehicle. In %particular, the OBU records sequences of positions during the %movement of the vehicle, as well as switching on and off, thus %memorizing the characteristics of the routes. The frequency of %recording the position of vehicles is currently programmed in two %ways: every 30 seconds when the vehicle is located along the %Italian motorway network or along some main roads located in %metropolitan areas, every 2 kilometers traveled in remaining %cases. %The GPS receiver identifies the position of the vehicle in the WGS84 Geographic Reference System. The GPS receiver associates the position with the date and time at the Greenwich meridian, the instantaneous speed and the direction of the vehicle mark expressed in degrees with respect to the geographic North. 
%    The dataset collects the travel trajectories in 2015 from October %31 to November 30. The last 7 days were used as a test set, while %the other days constitute the train set. The length of each time %period is set to one hour and 30 minutes.
\end{enumerate}
\stefano{
The Beijing dataset and New York Bike dataset are available on  %\textit{OneDrive}\footnote{\url{https://onedrive.live.com/?authkey=\%21ALcGog0cuaA1SLo&id=66E5DE6FBC377A48\%2178914&cid=66E5DE6FBC377A48}} 
\cite{Zhang2018} Github repository, already structured to carry out the experiments.}
Instead, for what regards the two datasets, New York Taxi was first downloaded from the \textit{NYC government website}\footnote{\url{https://www1.nyc.gov/site/tlc/about/tlc-trip-record-data.page}}, and later structured to carry out the experiments. %The first was downloaded from  while the second was provided to us by \textit{ENEA (National Agency for New Technologies, Energy and Sustainable Economic Development)}.
\vin{perché hai scelto questi dataset? perché mi hai riportato i periodi esatti di acquisizione dati? non bastava dire 3 mesi, 4 mesi, ecc.? che impatto ha sull'esperimento il fatto che tu stia considerando città diverse, mezzi di trasporto differenti, stagioni diverse (se usi meteo e fai training a dicembre, non mi aspetto una gran previsione a luglio). Questi sono i fattori che devi discutere qui}
